HierarchyNet: Learning to Summarize Source Code with Heterogeneous Representations

We propose a novel method for code summarization utilizing Heterogeneous Code Representations (HCRs) and our specially designed HierarchyNet. HCRs effectively capture essential code features at lexical, syntactic, and semantic levels by abstracting coarse-grained code elements and incorporating fine-grained program elements in a hierarchical structure. Our HierarchyNet method processes each layer of the HCR separately through a unique combination of the Heterogeneous Graph Transformer, a Tree-based CNN, and a Transformer Encoder. This approach preserves dependencies between code elements and captures relations through a novel Hierarchical-Aware Cross Attention layer. Our method surpasses current state-of-the-art techniques, such as PA-Former, CAST, and NeuralCodeSum.

==> applications.tex <==
%!TEX root=acl2023.tex




==> discussion.tex <==
%!TEX root=acl2023.tex
%Here, we will cover other parts of our framework. By using Code Hierarchy, we modify how code is often represented (as a graph or tree), which somewhat solves the over-squashing issue \cite{alon2021oversquashing} in "GNNs for code". The Code Hierarchy reduces the size of a AST by moving a large number of nodes from the AST-level to the Subtree-level rather than keeping the code as a graph as in earlier work \cite{Allamanis2018, wang2020learning}. This will make the HGT’s message-passing steps on the AST-level easier. Through our evaluations, we have shown that \methodname outperforms a few GNNs methods in different tasks. It shows that our model has the potential to address the over-squashing issue of the GNNs model of code. In fact, while in-depth analysis of this problem is not the primary focus of our paper, it is an interesting area for future research. Similar to \citet{alon2021oversquashing}, we plan to perform additional analysis to fully assess our framework, with a focus on the over-squashing issue of GNN models of code on the Code Hierarchy. Moreover, our framework is adaptable, allowing us to pretrain the model using a variety of strategies, such as predicting missing  edges~\cite{guo2020graphcodebert}, predicting missing variables~\cite{wang2021codet5}, predicting natural language descriptions~\cite{wang2021codet5}, etc. Such pretraining strategies can also be applied to our framework easily. In the future, we hope to create a unified pretraining framework that includes various types of pretraining tasks on top of Code Hierarchy. 

% Another potential extension of our work is to design a learning algorithm for clustering nodes in each level of granularity in a fully data-driven manner. This extension allows us to completely replace the current human-engineered coarse-graining procedure and add more flexibility for the model to discover the optimal clustering at each level and build a deeper hierarchy.

%For model explainability, in line with our work, there are many previous works that attempt to explain the output of source code models, including AutoFocus~\cite{bui2019autofocus} and SIVAND~\cite{rabin2021understanding}. They either use attention scores or simplify programs to remove redundant parts of source code for explainability. However, it is unknown whether such explanations are aligned with how developers understand code, which we believe is critical for the explainability on source code models. Extensive research on human evaluation is required to achieve this, but it is not the primary focus of our work. 

==> motivation.tex <==
In this section, we present the revolutions of code and our motivation behind Code Hierarchy. As source code is strictly in line with programming language grammars, a common practice ís to utilize Abstract Syntax Tree to encode the structural information of the code. However
